Diverse Weight Averaging for Out-of-Distribution Generalization

Standard neural networks struggle to generalize under distribution shifts in computer vision. Fortunately, combining multiple networks can consistently improve out-of-distribution generalization. In particular, weight averaging (WA) strategies were shown to perform best on the competitive DomainBed benchmark; they directly average the weights of multiple networks despite their nonlinearities. In this paper, we propose Diverse Weight Averaging (DiWA), a new WA strategy whose main motivation is to increase the functional diversity across averaged models. To this end, DiWA averages weights obtained from several independent training runs: indeed, models obtained from different runs are more diverse than those collected along a single run thanks to differences in hyperparameters and training procedures. We motivate the need for diversity by a new bias-variance-covariance-locality decomposition of the expected error, exploiting similarities between WA and standard functional ensembling. Moreover, this decomposition highlights that WA succeeds when the variance term dominates, which we show occurs when the marginal distribution changes at test time. Experimentally, DiWA consistently improves the state of the art on DomainBed without inference overhead.

==> tables/domainbed/db_home0_dwa_of_ma.tex <==
% {e0_acc_net: 66.3, e0_acc_netm: 59.3, e0_acc_soup: 66.9, e0_acc_soupswa: 67.2, e0_acc_swa: 67.2, e0_acc_swam: 65.4, gpu: 0, length: 40}
% {e0_acc_net: 66.2, e0_acc_netm: 59.0, e0_acc_soup: 68.0, e0_acc_soupswa: 67.6, e0_acc_swa: 67.2, e0_acc_swam: 65.6, gpu: 0, length: 40}
% {e0_acc_net: 66.0, e0_acc_netm: 60.6, e0_acc_soup: 67.2, e0_acc_soupswa: 66.3, e0_acc_swa: 65.9, e0_acc_swam: 64.5, gpu: 0, length: 40}
% {e0_acc_net: 66.7, e0_acc_netm: 59.6, e0_acc_soup: 68.2, e0_acc_soupswa: 67.5, e0_acc_swa: 66.9, e0_acc_swam: 65.1, gpu: 0, length: 120}

\begin{table}[h]%
    \caption{\textbf{DiWA vs MA} are complementary in OfficeHome domain `Art`.}
    \centering
    \adjustbox{width=0.7\textwidth}{
        \begin{tabular}{lccc}
            \toprule
            \textbf{Algorithm}               & \textbf{Weights selection} & \textbf{$M=20$} & \textbf{$M=60$} \\
            \midrule
            ERM                              & N/A                        & 62.9 $\pm$ 1.3                    \\
            MA                               & Uniform $M=4900$           & 65.0 $\pm$ 0.2                    \\
            \midrule
            DiWA                              & Uniform: $M=20$            & 67.3 $\pm$ 0.2                    \\
            DiWA$^{\dagger}$                  & Uniform: $M=60$            & 67.7
            \midrule
            DiWA of MA                        & Uniform: $M=20\times 4900$ & 66.7 $\pm$ 0.4                    \\
            DiWA$^{\dagger}$ of MA            & Uniform: $M=60\times 4900$ & 67.3                              \\
            \midrule
            DiWA of best and last             & Uniform: $M=20\times 2$    & 67.4 $\pm$ 0.3                    \\
            DiWA$^{\dagger}$ of best and last & Uniform: $M=60\times 2$    & 68.2                              \\
            \bottomrule
        \end{tabular}}
    \label{table:db_home0_dwa_of_ma}%
\end{table}


% {e0_acc_net: 66.4, e0_acc_netm: 59.9, e0_acc_soup: 67.5, e0_acc_soupswa: 66.8, e0_acc_swa: 67.2, e0_acc_swam: 65.1, gpu: 0, length: 20}
% {e0_acc_net: 65.9, e0_acc_netm: 59.5, e0_acc_soup: 67.7, e0_acc_soupswa: 67.4, e0_acc_swa: 67.0, e0_acc_swam: 65.5, gpu: 0, length: 20}
% {e0_acc_net: 66.0, e0_acc_netm: 60.9, e0_acc_soup: 66.9, e0_acc_soupswa: 65.8, e0_acc_swa: 65.6, e0_acc_swam: 64.3, gpu: 0, length: 20}
% {e0_acc_net: 66.5, e0_acc_netm: 60.1, e0_acc_soup: 67.7, e0_acc_soupswa: 67.3, e0_acc_swa: 66.7, e0_acc_swam: 65.0, gpu: 0, length: 60}


==> tables/domainbed/db_main_officehome0.tex <==
\begin{table}[h]%
  \caption{\textbf{Averaging different objectives on OfficeHome domain "Art"}.}%
  \centering%
  \adjustbox{width=0.7\textwidth}{%
    \begin{tabular}{lcccc}%
      \toprule
      \textbf{Algorithm} & \textbf{SGD}               & \textbf{MA} \cite{arpit2021ensemble} & \textbf{DiWA Uniform} $M=20$       & \textbf{DiWA$^{\dagger}$ Uniform}: $M=60$ \\
      \midrule
      ERM                & 62.9 $\pm$ 1.3             & \underline{65.0} $\pm$ 0.2           & 67.3 $\pm$ 0.2             & 67.7                             \\
      Mixup              & \underline{63.1} $\pm$ 0.7 & \textbf{66.2} $\pm$ 0.3              & 67.8 $\pm$ 0.6             & 68.4                             \\
      Coral              & \textbf{64.4} $\pm$ 0.4    & 64.4 $\pm$ 0.4                       & 67.7 $\pm$ 0.2             & 68.2                             \\
      ERM/Mixup          & N/A                        & N/A                                  & 67.9 $\pm$ 0.7             & \underline{68.9}                 \\
      ERM/Coral          & N/A                        & N/A                                  & \underline{68.1} $\pm$ 0.3 & 68.7                             \\
      ERM/Mixup/Coral    & N/A                        & N/A                                  & \textbf{68.4} $\pm$ 0.4    & \textbf{69.1}                    \\
      \bottomrule
    \end{tabular}}
  \label{table:db_home0_training}%
\end{table}

